Tracking Noisy Targets: A Review of Recent Object Tracking Approaches

Visual object tracking is an important computer vision problem with numerous real-world applications including human-computer interaction, autonomous vehicles, robotics, motion-based recognition, video indexing, surveillance and security. In this paper, we aim to extensively review the latest trends and advances in the tracking algorithms and evaluate the robustness of trackers in the presence of noise. The first part of this work comprises a comprehensive survey of recently proposed tracking algorithms. We broadly categorize trackers into correlation filter based trackers and the others as non-correlation filter trackers. Each category is further classified into various types of trackers based on the architecture of the tracking mechanism. In the second part of this work, we experimentally evaluate tracking algorithms for robustness in the presence of additive white Gaussian noise. Multiple levels of additive noise are added to the Object Tracking Benchmark (OTB) 2015, and the precision and success rates of the tracking algorithms are evaluated. Some algorithms suffered more performance degradation than others, which brings to light a previously unexplored aspect of the tracking algorithms. The relative rank of the algorithms based on their performance on benchmark datasets may change in the presence of noise. Our study concludes that no single tracker is able to achieve the same efficiency in the presence of noise as under noise-free conditions; thus, there is a need to include a parameter for robustness to noise when evaluating newly proposed tracking algorithms.

==> hierarchyV1.tex <==
\section{Classifications of Tracking Algorithms}

\begin{figure}
\centering
\includegraphics[width=10 cm]{./figures/Hierarichy.pdf}
\caption{Hierarchy of tracking algorithms}
\label{Hier1}
\end{figure}


We have studied 20 different tracking algorithms and each algorithm is to solve one or more tracking challenges. Different tracking algorithms involves different methods to exploit target structure for prediction of target location in a sequence. By analyzing and understanding the tracking procedure of selected trackers, we made a hierarchy to classify trackers into a specific type based upon their approaches. We have classified the tracking algorithms as correlation filter (CF) and non-correlation filter (Non-CF)  trackers. 

\subsection{Correlation Filter Trackers}
Correlation filter based tracking schemes perform computation in frequency domain to handle computational cost. During the tracking of general correlation filter based trackers, image patch is cropped on current frame based on the estimated target location on previous frame. Better description is defined by extraction of input feature map. In CF trackers, window boundaries are smoothed by applying cosine window. Response map is computed in element-wise manner by applying learned correlation filters in frequency domain. Inverse Fast Fourier Transform (IFFT) is applied over response map to obtain spatial confidence map. New target position is estimated at the maximum confidence score. At the end, target appearance at newly predicted location is trained by extracting features and updating correlation filters.

CF based trackers are further divided into three categories as CF, correlation operators and Siame trackers. CF trackers are just like general correlation filter based trackers including different feature extraction methods or play sufficient role of correlation filters to estimate targets. Correlation operators are special form of correlation filters where geometric structure of target is exploited using specialized correlation operators. Siame correlation trackers as clear from the same that they find similarities between two patches using correlation filters.


\subsection{Non-Correlation Filter Trackers}

There are many trackers which do not apply correlation filters for tracking are categorized as non-correlation trackers. Those trackers either explore the inner structure of target or track object by learning image patches. Based on these properties, non-CF are categorized as target template and patch learning trackers. In target template tracking methods, appearance of target is exploited in the first frame of the sequence and tracking is performed on the rest of the frames. while in patch learning, object and background patches are trained to estimate the target in new frame.
